An equilibrium approach to modelling social interaction

The aim of this work is to put forward a statistical mechanics theory of social interaction, generalizing econometric discrete choice models. After showing the formal equivalence linking econometric multinomial logit models to equilibrium statical mechanics, a multi-population generalization of the Curie-Weiss model for ferromagnets is considered as a starting point in developing a model capable of describing sudden shifts in aggregate human behaviour. Existence of the thermodynamic limit for the model is shown by an asymptotic sub-additivity method and factorization of correlation functions is proved almost everywhere. The exact solution of the model is provided in the thermodynamical limit by finding converging upper and lower bounds for the system's pressure, and the solution is used to prove an analytic result regarding the number of possible equilibrium states of a two-population system. The work stresses the importance of linking regimes predicted by the model to real phenomena, and to this end it proposes two possible procedures to estimate the model's parameters starting from micro-level data. These are applied to three case studies based on census type data: though these studies are found to be ultimately inconclusive on an empirical level, considerations are drawn that encourage further refinements of the chosen modelling approach.

==> capitolo_final_remarks.tex <==

\resettheoremcounters

\chapter{Final remarks}

%In this paper we deepen the bridge among statistical mechanics and
%social sciences with particular emphasis on the statistical tools
%for comparison among theoretical models and real data when peer interaction plays a considerable role.
%\newline
We introduced a class of simple mean field models of choice in the
presence of social interaction, which generalizes
the model introduced in \cite{durlauf}.
%standard non-linear regression when the interaction parameters are set
%to zero (as the Discrete Choice theory), as well as for the interaction
%among social agents inside coarse grained sector of society, whose
%size is ultimately suggested by the amount of linear regressors
%themselves.

After showing how our model reduces to a standard discrete choice model
when we neglect interaction, we analyzed the simplest kind of interaction
(by accounting for only one attribute): in this case the model reduces to
a well known bipartite model, whose thermodynamic limit as well as
multiple equilibria have already been shown to exist \cite{gaco}.
\newline
In order to test our model we considered three case studies, concerning
relevant social phenomena such as marriage, divorce, and suicide, and we
found that Berkson's method of estimation \cite{berkson} provides
a valuable statistical tool, alternative to the more typical maximum likelihood procedure
used in econometrics, which is not suitable for our model due to discontinuities
arising in its probability structure.
\newline
%This papers aims to suggest the outline of a method that can be used to study more specific
%situations, where individuals may be modelled in a more precise way, by assigning
%more socio-economic attributes to them. In this simple case we were able to find
% consistencies in the interaction parameters regarding different topics for the
% same population.  Furthermore, the parameters values where found to be in a regime
% characterized by multiple equilibria, which suggests the possibility that a
% refinement of this study will eventually lead to the capability of predicting
% abrupt transitions at a societal level.
